Towards Query Logs for Privacy Studies: On Deriving Search Queries from Questions

Translating verbose information needs into crisp search queries is a phenomenon that is ubiquitous but hardly understood. Insights into this process could be valuable in several applications, including synthesizing large privacy-friendly query logs from public Web sources which are readily available to the academic research community. In this work, we take a step towards understanding query formulation by tapping into the rich potential of community question answering (CQA) forums. Specifically, we sample natural language (NL) questions spanning diverse themes from the Stack Exchange platform, and conduct a large-scale conversion experiment where crowdworkers submit search queries they would use when looking for equivalent information. We provide a careful analysis of this data, accounting for possible sources of bias during conversion, along with insights into user-specific linguistic patterns and search behaviors. We release a dataset of 7,000 question-query pairs from this study to facilitate further research on query understanding.

==> sections/discussion.tex <==
\section{Discussion - TODO}
\label{sec:discuss}

%\textbf{Training-dev-test split.} In 60:20:20. Split preserves profile length distribution.

%\textbf{For methods that use clicks.} Several methods use click information as a key component.
%Methods with clicks may be applied as follows, a suggestion.
%Clicks are implicit judgments.
%Answers as notion of pseudo-relevance feedback. 1 in 3-point scale.
%Last click, assumed to be most relevant - here the accepted answer (rating 2). Other clicks are the documents with 1-point rating. More to follow (upvotes and downvotes?).

\textbf{Usefulness in other tasks.} Our detailed profiles will help in tasks other in ranking. Personalized query expansion, query autocompletion, query suggestion. 

Only adopt query length distribution from AOL log. No violation of privacy.

%\textbf{Question to Answer propagation.} The problem with the documents as answers - they might only implicitly contain the vocabulary of the question. Propagate the questions to answers?

\textbf{Limitations.}
Only topical queries - personalization algos can only be tested accordingly . No sensitive/identifying information; in practice, personalization might need to be applied over such items (locations, names, numbers, etc...) However, a large body of work explicitly focuses on personalization of topical queries, even though there's some auditing work that shows personalization is being applied over non-topical items.

\textbf{Query reduction techniques.}
 longer queries ina real setup tend to have more low-idf words,  in our case, the long queries are just a chain of informative words.
 "mail imap exising server domain provider exchange backup active". the length of the query should perhaps also depend somehow on the length of the question instead of being randomly chosen for each question?
 
 

==> sections/query_conversion.tex <==
\section{Automatic conversion from questions to queries}
\label{sec:query-conversion}

\subsection{Problem statement.}


\subsection{Features.}


\subsection{Baselines.}


\subsection{Learning to rank question words.}


\subsection{Global and user specific models.}


\subsection{Data.}
Format of the inputs, size, 


\subsection{Results and insights.}



==> sections/userstudy-anecdotal.tex <==
\subsection{Anecdotal results.}





==> sections/userstudy-personalization.tex <==
\subsection{Personalization / Personal differences}
\abcomment{Do we even go into explaining this? could be a nice add on showing that individual differences matter}

Tasks in our study were composed of multiple questions,
so as to gather the information on how different people tend to construct queries.
We validate whether there are individual differences in query formulation as follows.
We train a learning-to-rank model to rank the questions words such that the top-ones
correspond to query words. The training data consists of sets of rankings (=questions),
with the relevance being the binary information on whether the word ended up in the corresponding query.
We first train a global model where...
Then we train a number of personalized models ...
We see am improvement in the effectiveness of the personalized model,
showing that individual differences do exist...
